Motion Inspired Unsupervised Perception and Prediction in Autonomous Driving

Learning-based perception and prediction modules in modern autonomous driving systems typically rely on expensive human annotation and are designed to perceive only a handful of predefined object categories. This closed-set paradigm is insufficient for the safety-critical autonomous driving task, where the autonomous vehicle needs to process arbitrarily many types of traffic participants and their motion behaviors in a highly dynamic world. To address this difficulty, this paper pioneers a novel and challenging direction, i.e., training perception and prediction models to understand open-set moving objects, with no human supervision. Our proposed framework uses self-learned flow to trigger an automated meta labeling pipeline to achieve automatic supervision. 3D detection experiments on the Waymo Open Dataset show that our method significantly outperforms classical unsupervised approaches and is even competitive to the counterpart with supervised scene flow. We further show that our approach generates highly promising results in open-set 3D detection and trajectory prediction, confirming its potential in closing the safety gap of fully supervised systems.

==> defs.tex <==
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\etal{\emph{et al}\onedot}
\def\eg{\emph{e.g}\onedot}
\def\etc{\emph{etc}\onedot}
\def\ie{\emph{i.e}\onedot}
\def\dbscan{DBSCAN\xspace}

\def\@fnsymbol#1{\ensuremath{\ifcase#1\or *\or \dagger\or \ddagger\or
   \mathsection\or \mathparagraph\or \|\or **\or \dagger\dagger
   \or \ddagger\ddagger \else\@ctrerr\fi}}
\newcommand*\samethanks[1][\value{footnote}]{\footnotemark[#1]}

\crefname{section}{Sec.}{Secs.}
\Crefname{section}{Section}{Sections}
\Crefname{table}{Table}{Tables}
\crefname{table}{Tab.}{Tabs.}

\newcommand{\cutsectionup}{\vspace*{-10pt}}
\newcommand{\cutsectiondown}{\vspace*{-4pt}}
\newcommand{\cutsubsectionup}{\vspace*{-8pt}}
\newcommand{\cutsubsectiondown}{\vspace*{-2pt}}
\newcommand{\cutsubsubsectionup}{\vspace*{-0pt}}
\newcommand{\cutsubsubsectiondown}{\vspace*{-0pt}}
\newcommand{\cutparagraphup}{\vspace*{-6pt}}
\newcommand{\cutparagraphdown}{\vspace*{-0pt}}
\newcommand{\cuthalfcaptionup}{\vspace*{-0pt}}
\newcommand{\cuthalfcaptiondown}{\vspace*{-5pt}}
\newcommand{\cutcaptionup}{\vspace*{-10pt}}
\newcommand{\cutcaptiondown}{\vspace*{-10pt}}
\newcommand{\cuthalftablecaptionup}{\vspace*{-5pt}}
\newcommand{\cuthalftablecaptiondown}{\vspace*{-0pt}}
\newcommand{\cuttablecaptionup}{\vspace*{-0pt}}
\newcommand{\cuttablecaptiondown}{\vspace*{-0pt}}
\newcommand{\cutequationup}{\vspace*{-0pt}}
\newcommand{\cutequationdown}{\vspace*{-0pt}}
\newcommand{\cuthalftableup}{\vspace*{-0pt}}
\newcommand{\cuthalftabledown}{\vspace*{-0pt}}
\newcommand{\cuttableup}{\vspace*{-0pt}}
\newcommand{\cuttabledown}{\vspace*{-0pt}}
\newcommand{\cutabstractup}{\vspace*{-0pt}}
\newcommand{\cutabstractdown}{\vspace*{-0pt}}
\newcommand{\cut}{{\vspace*{-0in}}}
\newcommand{\cutmore}{{\vspace*{-0in}}}
\newcommand{\negcut}{}
